Complex-valued embeddings of generic proximity data

Proximities are at the heart of almost all machine learning methods. If the input data are given as numerical vectors of equal lengths, euclidean distance, or a Hilbertian inner product is frequently used in modeling algorithms. In a more generic view, objects are compared by a (symmetric) similarity or dissimilarity measure, which may not obey particular mathematical properties. This renders many machine learning methods invalid, leading to convergence problems and the loss of guarantees, like generalization bounds. In many cases, the preferred dissimilarity measure is not metric, like the earth mover distance, or the similarity measure may not be a simple inner product in a Hilbert space but in its generalization a Krein space. If the input data are non-vectorial, like text sequences, proximity-based learning is used or ngram embedding techniques can be applied. Standard embeddings lead to the desired fixed-length vector encoding, but are costly and have substantial limitations in preserving the original data's full information. As an information preserving alternative, we propose a complex-valued vector embedding of proximity data. This allows suitable machine learning algorithms to use these fixed-length, complex-valued vectors for further processing. The complex-valued data can serve as an input to complex-valued machine learning algorithms. In particular, we address supervised learning and use extensions of prototype-based learning. The proposed approach is evaluated on a variety of standard benchmarks and shows strong performance compared to traditional techniques in processing non-metric or non-psd proximity data.

==> 01_Preamble/Floating-AND-TOC-AND-ListOf-AND-Headings.tex <==
%%% File encoding is ISO-8859-1 (also known as Latin-1)
%%% You can use special characters just like ä,ü and ñ

% ##############################################
% Start: Table of Contents (TOC) Customization
% ##############################################
%

% Level for numbered captions
\setcounter{secnumdepth}{5}

% Level of chapters that appear in Table of Contents
\setcounter{tocdepth}{5} % bis wohin ins Inhaltsverzeichnis aufnehmen
% -2 no caption at all
% -1 part
% 0  chapter
% 1  section    
% 2  subsection 
% 3  subsubsection
% 4  paragraph
% 5  subparagraph

% KOMA-Script code to adjust TOC
% Applying the color 'myColorMainA' which is defined in the main file (MainFile.tex)
\makeatletter
\addtokomafont{chapterentrypagenumber}{\color{myColorMainA}}
\addtokomafont{chapterentry}{\color{myColorMainA}}
\makeatother

%
% #######################
% End: Table of Contents (TOC) Customization
% #######################

% ##############################################
% Start: Floating Object Customization
% ##############################################
%

% Extended support for catioons of figures and tables etc.
% CTAN: http://www.ctan.org/pkg/caption
\usepackage[%
	font={small},
	labelfont={bf,sf},
	format=hang, % try plain or hang
	margin=5pt,
]{caption}
%

% #######################
% End: Floating Object Customization
% #######################

% ##############################################
% Start: Headings Customization
% ##############################################
%

% KOMA-Script code to customize the headings
% Applying the color 'myColorMainA' which is defined in the main file (MainFile.tex)
\addtokomafont{chapter}{\color{myColorMainA}}
\addtokomafont{section}{\color{myColorMainA}}
\addtokomafont{subsection}{\color{myColorMainA}}
\addtokomafont{subsubsection}{\color{myColorMainA}}
\addtokomafont{paragraph}{\color{myColorMainA}}
\addtokomafont{subparagraph}{\color{myColorMainA}}

% #######################
% End: Headings Customization
% #######################


==> 01_Preamble/HeaderFooterMarginnote.tex <==
%%% File encoding is ISO-8859-1 (also known as Latin-1)
%%% You can use special characters just like ä,ü and ñ

% Custom command fpr the margin notes: \myMarginnote{Your Text}
% Comment on the \lineskiplimit=-\maxdimen:
% See http://tex.stackexchange.com/questions/49072/
% Without it the line spacing of the normal text was changed (ugly).
\newcommand{\myMarginnote}[1]{%
	\marginnote{% needs marginnote package
		\ifthispageodd{\RaggedRight}{\RaggedLeft}% needs ragged2e package
		\color{myColorMainB}%
		\lineskiplimit=-\maxdimen% 
		\normalfont\sffamily\scriptsize%
		#1}%
}

% ##############################################
% Start: Header and Footer Customization
% ##############################################
%

% KOMA-Script code for header and footer font
\setkomafont{pageheadfoot}{%
	\normalfont\sffamily\bfseries
	}
\setkomafont{pagefoot}{%
	\normalfont\sffamily
	}
\setkomafont{pagenumber}{%
	\normalfont\rmfamily
	}

% Define width of header
\setheadwidth[0pt]{textwithmarginpar}

% Define with of header line
\setheadsepline{0.4pt}

% Define width of footer
\setfootwidth[0pt]{text}
% Define with of footer line (here: no line)
\setfootsepline[text]{0pt}

% Some calculations
% calc package is needed which is loaded here: 01_Preamble/CommonPackages.tex
% If you want to understand the calculations visit:
% http://en.wikibooks.org/wiki/LaTeX/Page_Layout
\newlength{\myLenghthFootAbstand}
\setlength{\myLenghthFootAbstand}{\paperheight-1in-\topmargin- \headheight-\headsep-\textheight-\footskip}
\newlength{\myLenghthTemp}
\setlength{\myLenghthTemp}{\myLenghthFootAbstand+\baselineskip}

% Define content of header and footer
% Using some scrpage2 commands here. The scrpage2 package is loaded here: 01_Preamble/KOMA-Script-Packages.tex
% Some LaTeX magic...
% Clear all defaults
\clearscrheadfoot
% Header
\ohead{%
	\textcolor{myColorMainA}{\headmark}
	}
% Left (even page numbers) footer
\lefoot%
[% scrplain style (begin)
	\setlength{\unitlength}{\myLenghthFootAbstand}%
	\begin{picture}(0,0)%
		\put(0,-1)%
		{%
			\makebox(0,0)[lb]%
			{%
				\rule{0.4pt}{\myLenghthTemp}%
			}%
		}%
	\end{picture}\llap{\pagemark~}%
]% scrplain style (end)
%
{% scrheadings style (begin)
	\setlength{\unitlength}{\myLenghthFootAbstand}%
	\begin{picture}(0,0)%
		\put(0,-1)%
		{%
			\makebox(0,0)[lb]%
			{%
				\rule{0.4pt}{\myLenghthTemp}%
			}%
		}%
	\end{picture}\llap{\pagemark~}%
}% scrheadings style (end)

% Right (odd page numbers) footer
\rofoot%
[% scrplain style (begin)
	\rlap{~\pagemark}%%
	\setlength{\unitlength}{\myLenghthFootAbstand}%
	\begin{picture}(0,0)%
		\put(0,-1)%
		{%
			\makebox(0,0)[lb]%
			{%
				\rule{0.4pt}{\myLenghthTemp}%
			}%
		}%
	\end{picture}%
]% scrplain style (end)
%
{% scrplain style (begin)
	\rlap{~\pagemark}%%
	\setlength{\unitlength}{\myLenghthFootAbstand}%
	\begin{picture}(0,0)%
		\put(0,-1)%
		{%
			\makebox(0,0)[lb]%
			{%
				\rule{0.4pt}{\myLenghthTemp}%
			}%
		}%
	\end{picture}%
}% scrplain style (end)

%
% #######################
% End: Header and Footer Customization
% #######################

==> 01_Preamble/KOMA-Script-Packages.tex <==
%%% File encoding is ISO-8859-1 (also known as Latin-1)
%%% You can use special characters just like ä,ü and ñ

% Special KOMA-Script package - I added it because I also use the float package in this template, see: 
% http://tex.stackexchange.com/questions/51867/koma-warning-about-toc
% CTAN: http://www.ctan.org/tex-archive/macros/latex/contrib/koma-script/doc
\usepackage{scrhack}

% Better support for marginnotes
% new command: \marginnote
% LaTeX standard command: \marginpar
% CTAN: http://www.ctan.org/pkg/marginnote
\usepackage{marginnote}

% Extended header and footer support
% CTAN: http://www.ctan.org/pkg/scrpage2
\usepackage[%
  	automark
  	,ilines
	,headsepline
	,footsepline
]{scrpage2}

==> 01_Preamble/PDF-Related.tex <==
%%% File encoding is ISO-8859-1 (also known as Latin-1)
%%% You can use special characters just like ä,ü and ñ

% Package for PDF features such as bookmarks and hyperlinks. 
% Important: Should be loaded at the end.
% CTAN: http://www.ctan.org/pkg/hyperref
\usepackage[%
bookmarks, % Create bookmarks
bookmarksopen=true, % Unfold bookmatk tree in PDF viewer when document is opened
bookmarksopenlevel=1, % Level of unfolding
bookmarksnumbered=true, % Number bookmarks
hidelinks, % do not highlight hyperlinks -- looks ugly
% Ansicht beim Öffnen
pdfpagelabels=true, % See manual...
plainpages=false, % See manual...
hyperfootnotes=true, % Hyperlinks for footnotes
hyperindex=true, % Indexeinträage verweisen auf Text
]{hyperref}

==> 01_Preamble/PageLayout.tex <==
%%% File encoding is ISO-8859-1 (also known as Latin-1)
%%% You can use special characters just like ä,ü and ñ

% User friendly interface to change layout parameters
% CTAN: http://www.ctan.org/pkg/geometry
\usepackage{geometry}
\geometry{% siehe geometry.pdf (Figure 1)
	bottom=30mm,
	showframe=false, % For debugging: try true and see the layout frames
	margin=30mm,
	marginparsep=3mm,
	marginparwidth=20mm
}

==> 01_Preamble/ParagraphOptimization.tex <==
%%% File encoding is ISO-8859-1 (also known as Latin-1)
%%% You can use special characters just like ä,ü and ñ

% This is an suggestion from Axel Reichert (LaTeX package author)
% See CTAN: http://www.ctan.org/author/reichert
% See CTAN: http://www.ctan.org/pkg/l2tabu-english (Cgapter: 1.8 Should I use \sloppy?)

\tolerance 1414
\hbadness 1414
\emergencystretch 1.5em
\hfuzz 0.3pt
\widowpenalty=10000
\vfuzz \hfuzz
\raggedbottom

==> 01_Preamble/documentclass.tex <==
%%% File encoding is ISO-8859-1 (also known as Latin-1)
%%% You can use special characters just like ä,ü and ñ

% KOMA-Script class 'scrbook'
% Link to the documentation: 
% German: http://mirrors.ctan.org/macros/latex/contrib/koma-script/doc/scrguide.pdf
% English: http://mirrors.ctan.org/macros/latex/contrib/koma-script/doc/scrguien.pdf
% CTAN: http://www.ctan.org/pkg/koma-script
% Author of the KOMA-Script family is Markus Kohm
\documentclass%
[%
paper=a4
,fontsize=11pt % common are 10, 11 or 12
,headings=big
,parskip
,numbers=noendperiod % 2.3.1 vs 2.3.1. (no dot after the last chapter number)
,oneside
,toc=bibliography % Bibliography appears in Table of Contents (without a number)
,toc=listof % List of Figures and List of Tables appear in Table of Contents
,version=last % Use latest version of the KOMA-Script
]%
{scrbook}
